Learning to Compile Programs to Neural Networks

A $\textit{neural surrogate of a program}$ is a neural network that mimics the behavior of a program. Researchers have used these neural surrogates to automatically tune program inputs, adapt programs to new settings, and accelerate computations. Researchers traditionally develop neural surrogates by training on input-output examples from a single program. Alternatively, language models trained on a large dataset including many programs can consume program text, to act as a neural surrogate. Using a language model to both generate a surrogate and act as a surrogate, however, leading to a trade-off between resource consumption and accuracy. We present $\textit{neural surrogate compilation}$, a technique for producing neural surrogates directly from program text without coupling neural surrogate generation and execution. We implement neural surrogate compilers using hypernetworks trained on a dataset of C programs and find that they produce neural surrogates that are $1.9$-$9.5\times$ as data-efficient, produce visual results that are $1.0$-$1.3\times$ more similar to ground truth, and train in $4.3$-$7.3\times$ fewer epochs than neural surrogates trained from scratch.

==> sections/denoising_results_extended.tex <==
\section{\textsc{CompNet} Improvements To Perceptual Quality (Extended)}\label{sec:denoising_results_extended}
In this section, we present end-to-end denoising results (see Section~\ref{sec:e2e_results}) for all dataset sizes we trained surrogates for in the data efficiency evaluation (see Section~\ref{sec:data_efficiency}).

The full listing of results is in Figure~\ref{fig:full_denoise_results}.
When there is no training data, none of the approximate implementations resemble the NumPy result.
However, when surrogates are trained on $0.1\%$ of the training data, \textsc{CompNet}s resemble the NumPy implementation most closely, with pretrained initializations a very close second.
All other approximate implementations are brighter than the NumPy result and/or include more prominent gridlines.
As the amount of data increases, other implementations close the gap and produce results on par with \textsc{CompNet}s.

\begin{figure*}
  \includegraphics[width=\textwidth]{figures/denoise/denoise_dataset_size_0_0.pdf}
  \includegraphics[width=\textwidth]{figures/denoise/denoise_dataset_size_0_001.pdf}
  \includegraphics[width=\textwidth]{figures/denoise/denoise_dataset_size_0_01.pdf}
  \includegraphics[width=\textwidth]{figures/denoise/denoise_dataset_size_0_1.pdf}
  \includegraphics[width=\textwidth]{figures/denoise/denoise_dataset_size_1_0.pdf}
  % \includegraphics{figures/denoise/denoise_dataset_size_0_001}
  \caption{
    End-to-end comparisons of neural surrogates produced by various initialization methods on a denoising task.
    In each row, the original noisy image is on the left, approximately denoised images using each initialization method are in the middle, and a ground-truth denoised image using an exact NumPy implementation is on the right.
  }\label{fig:full_denoise_results}
\end{figure*}


==> sections/lit_review.tex <==
\section{Literature Review}
\paragraph{Parrot.}
They identify that the requirement of fixed-size data and function purity have been identified as important for neural surrogate modeling~\cite{Parrot2012}. % End of Section 3.1
They say more accuracy could be gained by more intelligently sampling inputs. % Section 4.1
Table 1 gives a good suite of benchmarks to test against---not many functions in total though.

\paragraph{CPU Design Space Simulator.}
\cite{DesignSpaceNeuralSurrogate2006} develop a neural surrogate of a cycle-accurate simulator for evaluating architectural design choices.
They mention the impact of hyperparameter choices on quality in Section 2.1, the impact of input encodings in Section 2.3, and the impact of intelligent data sampling in Section 2.4.

\paragraph{DiffTune.}
They beef up Ithemal a bit and use the resulting surrogate for input optimization.
They don't really highlight the difficulties of the methodology here, because they're just using random inputs.

\paragraph{Neuzz.}
It looks like they're building a surrogate model of programs at the byte level, and it predicts which edges will be taken by a given input byte sequence.
They then use it to generate inputs that hit certain edges?
Doesn't seem like there's much that's highlighting the difficulty of neural surrogate methodology.
Maybe there's something about it being unclear at what level to model your problem at, since they make this weird choice of byte-level encoding?
Also, where are they getting their inputs?
They use existing evolutionary fuzzers like AFL to generate inputs for their model (NN Training part of Section IV) or existing test inputs (top of Section III).

\paragraph{Injection Molding Surrogate Adaptation.} \cite{InjectionMoldingSurrogateAdaptation2018} 
They had to do some hyperparameter search (Section 4).
They also considered a methodological dichotomy of directly adapting the pretrained surrogate to real data or first adding some new layers to the pretrained model, with the hypothesis being that real data is more complex and the network therefore needs more capacity.
Their evaluation seems kind of weird.
They compare a network trained from scratch on real data to the two network types listed above, but they only show those results for the training set.

\paragraph{Neural Surrogates For ISP Parameter Tuning.}
\cite{DiffTuneForGraphics2019} does the same thing as DiffTune.
There are a bunch of knobs you need to tune for ISPs to get the best-looking output, given the raw input signal.
You train a surrogate, then optimize the parameters with SGD.
I'm not sure how they're grabbing inputs.
It seems like they have some input images they care about (the ones they would normally give to an expert?), then they sample hyperparameters to feed to the ISP?
They say ``the $M$ images and sampled hyperparameters''.

\section{Future Work}
Automatically choose the architecture too.


==> sections/parrot_benchmark_code.tex <==
% \section{\textsc{ParrotBenchCPN} Code}\label{sec:parrot_benchmark_code}
% We present the code used for \textsc{ParrotBenchCPN} in our evaluation (Section~\ref{sec:evaluation}), which we adapted from \textsc{ParrotBench} to be pointer-free.
% The code for the benchmarks is shown in Figures~\ref{fig:fft_code}, \ref{fig:invk2j_code}, \ref{fig:kmeans_code}, and \ref{fig:sobel_code}.

% \begin{figure*}
% \centering
% \begin{minipage}{0.45\textwidth}
% \begin{minted}{c}
% float fftSin_Output0(float x) {
%     return sin(-2 * 3.1415 * x);
% }

% float fftSin_Output1(float x) {
%     return cos(-2 * 3.1415 * x);
% }
% \end{minted}
% \end{minipage}
% \caption{Code for the \texttt{fft} benchmark in \textsc{ParrotBenchCPN}.}\label{fig:fft_code}
% \end{figure*}

% \begin{figure*}
% \centering
% \begin{minipage}{0.45\textwidth}
% \begin{minted}{c}
% float invk2j_Output0(float x, float y) {
%   float l1 = 0.5 ;
%   float l2 = 0.5 ;
%   float theta2 = (float)acos(
%     ((x * x) + (y * y) - (l1 * l1) - (l2 * l2)) /
%     (2 * l1 * l2)) ;
%   return (float)asin(
%     (y * (l1 + l2 * cos(theta2)) - x * l2 * sin(theta2)) /
%     (x * x + y * y)) ;
% }

% float invk2j_Output1(float x, float y) {
%   float l1 = 0.5 ;
%   float l2 = 0.5 ;
%   return (float)acos(
%     ((x * x) + (y * y) - (l1 * l1) - (l2 * l2)) /
%     (2 * l1 * l2)) ;
% }
% \end{minted}
% \end{minipage}
% \caption{Code for the \texttt{invk2j} benchmark in \textsc{ParrotBenchCPN}.}\label{fig:invk2j_code}
% \end{figure*}

% \begin{figure*}
% \centering
% \begin{minipage}{0.45\textwidth}
% \begin{minted}{c}
% float euclideanDistance(
%   float p_0, float p_1, float p_2,
%   float c1_0, float c1_1, float c1_2) {
%   float r;

%   r = 0;
%   r += (p_0 - c1_0) * (p_0 - c1_0);
%   r += (p_1 - c1_1) * (p_1 - c1_1);
%   r += (p_2 - c1_2) * (p_2 - c1_2);

%   return sqrt(r);
% }
% \end{minted}
% \end{minipage}
% \caption{Code for the \texttt{kmeans} benchmark in \textsc{ParrotBenchCPN}.}\label{fig:kmeans_code}
% \end{figure*}

% \begin{figure*}
% \centering
% \begin{minipage}{0.45\textwidth}
% \begin{minted}{c}
% float sobel(
%   float w00, float w01, float w02,
%   float w10, float w11, float w12,
%   float w20, float w21, float w22)
% {
%   float sx = 0.0;
%   sx += w00 * -1;
%   sx += w10 * 0;
%   sx += w20 * 1;
%   sx += w01 * -2;
%   sx += w11 * 0;
%   sx += w21 * 2;
%   sx += w02 * -1;
%   sx += w12 * 0;
%   sx += w22 * 1;

%   float sy = 0.0;
%   sy += w00 * -1;
%   sy += w10 * -2;
%   sy += w20 * -1;
%   sy += w01 * 0;
%   sy += w11 * 0;
%   sy += w21 * 0;
%   sy += w02 * 1;
%   sy += w12 * 2;
%   sy += w22 * 1;

%   float s = sqrt(sx * sx + sy * sy) ;
%   if (s >= (256 / sqrt(256 * 256 + 256 * 256)))
%     s = 255 / sqrt(256 * 256 + 256 * 256);
%   return s ;
% }
% \end{minted}
% \end{minipage}
% \caption{Code for the \texttt{sobel} benchmark in \textsc{ParrotBenchCPN}.}\label{fig:sobel_code}
% \end{figure*}


==> sections/training_time_extended.tex <==
% \section{Training Time Improvements (Extended)}\label{sec:training_time_extended}
% Here we collect additional figures for the training time evaluation (Section~\ref{sec:training_time}).
% We present the initial train losses, initial test lossses, and target test losses for both \textsc{ExeStackCPN} (Figure~\ref{fig:exestack_training_time_loss}) and \textsc{ParrotBenchCPN} (Figures~\ref{fig:parrot_training_time_initial_train_loss}, \ref{fig:parrot_training_time_initial_test_loss}, and \ref{fig:parrot_training_time_target_test_loss}).
% We also present the average finish epoch (Figure~\ref{fig:avg_finish_epoch_parrot}) for each initialization method and the number of timeouts (Figure~\ref{fig:num_timeouts_parrot}) on \textsc{ParrotBenchCPN} programs.

% \begin{figure*}
%   \centering
%   \includegraphics[width=0.7\linewidth]{figures/training_time/exestack_initial_train_loss_histogram.pdf}
%   \includegraphics[width=0.7\linewidth]{figures/training_time/exestack_initial_test_loss_histogram.pdf}
%   \includegraphics[width=0.7\linewidth]{figures/training_time/exestack_target_test_loss_histogram.pdf}
%   \caption{
%     Histogram of initial train losses (top) and initial test losses (bottom) for surrogats produced by each initialization method in the training time evaluation, as well as a histogram of the target test losses set by random initialization after training for $5{,}000$ epochs.
%     Losses are not averaged across instances of initialization methods and trials.
%     Note that both the $x$ and $y$ axes are log-scale.
%   }\label{fig:exestack_training_time_loss}
% \end{figure*}

% \begin{figure*}
%   \centering
%     \begin{tabular}{lllll}
%     \toprule
%     Program & CPN (0) & CPN (1) & CPN (2) & CPN \\
%     \midrule
%     \texttt{fft} & $0.48 \pm \num{1.81e-06}$ & $0.43 \pm \num{8.51e-06}$ & $2.94 \pm \num{6.80e-05}$ & $1.28 \pm 1.20$ \\
%     \texttt{invk2j} & $1.14 \pm \num{5.67e-04}$ & $1.90 \pm \num{8.89e-04}$ & $2.54 \pm \num{1.52e-03}$ & $1.86 \pm 0.58$ \\
%     \texttt{kmeans} & $0.12 \pm \num{1.44e-05}$ & $0.09 \pm \num{1.33e-05}$ & $0.08 \pm \num{1.20e-05}$ & $0.10 \pm 0.02$ \\
%     \texttt{sobel} & $0.09 \pm \num{3.62e-04}$ & $0.13 \pm \num{4.21e-04}$ & $0.17 \pm \num{3.72e-04}$ & $0.13 \pm 0.03$ \\
%     \bottomrule
%     \end{tabular}
    
%     \vspace{1em}
%     \begin{tabular}{lllll}
%     \toprule
%     Program & MAML (0) & MAML (1) & MAML (2) & MAML \\
%     \midrule
%     \texttt{fft} & $0.57 \pm 0.18$ & $0.59 \pm 0.19$ & $0.53 \pm 0.14$ & $0.56 \pm 0.16$ \\
%     \texttt{invk2j} & $2.08 \pm 0.64$ & $2.07 \pm 0.59$ & $2.02 \pm 0.56$ & $2.06 \pm 0.58$ \\
%     \texttt{kmeans} & $0.76 \pm 0.46$ & $0.64 \pm 0.38$ & $0.79 \pm 0.52$ & $0.73 \pm 0.44$ \\
%     \texttt{sobel} & $0.24 \pm 0.16$ & $0.18 \pm 0.12$ & $0.25 \pm 0.22$ & $0.22 \pm 0.17$ \\
%     \bottomrule
%     \end{tabular}
    
%     \vspace{1em}
%     \begin{tabular}{lllll}
%     \toprule
%     Program & PTS (0) & PTS (1) & PTS (2) & PTS \\
%     \midrule
%     \texttt{fft} & $0.83 \pm 0.07$ & $0.84 \pm 0.07$ & $0.84 \pm 0.07$ & $0.84 \pm 0.07$ \\
%     \texttt{invk2j} & $2.11 \pm 0.57$ & $2.10 \pm 0.56$ & $2.12 \pm 0.59$ & $2.11 \pm 0.55$ \\
%     \texttt{kmeans} & $0.10 \pm \num{1.92e-05}$ & $0.10 \pm \num{1.88e-05}$ & $0.10 \pm \num{1.87e-05}$ & $0.10 \pm \num{1.34e-03}$ \\
%     \texttt{sobel} & $0.18 \pm \num{4.37e-04}$ & $0.19 \pm \num{4.40e-04}$ & $0.19 \pm \num{4.43e-04}$ & $0.19 \pm \num{3.55e-03}$ \\
%     \bottomrule
%   \end{tabular}
%   \vspace{1em}

%   \begin{tabular}{ll}
%     \toprule
%     Program & RND \\
%     \midrule
%     \texttt{fft} & $0.64 \pm 0.35$ \\
%     \texttt{invk2j} & $2.37 \pm 0.80$ \\
%     \texttt{kmeans} & $0.24 \pm 0.25$ \\
%     \texttt{sobel} & $0.36 \pm 0.34$ \\
%     \bottomrule
%   \end{tabular}
%   \caption{
%     Average initial train loss on \textsc{ParrotBenchCPN} for surrogates produced by each initialization method.
%     We include a column for each instance of an initialization method (e.g., ``CPN (0)'' is only one of the \textsc{CompNet}s we trained) as well as a column that averages over each instance (e.g., ``CPN'' is an average over all \textsc{CompNet}s we trained).
%   }\label{fig:parrot_training_time_initial_train_loss}
% \end{figure*}

% \begin{figure*}
%   \centering
%     \begin{tabular}{lllll}
%     \toprule
%     Program & CPN (0) & CPN (1) & CPN (2) & CPN \\
%     \midrule
%     \texttt{fft} & $0.48 \pm \num{0.00e+00}$ & $0.42 \pm \num{0.00e+00}$ & $2.92 \pm \num{0.00e+00}$ & $1.27 \pm 1.18$ \\
%     \texttt{invk2j} & $1.14 \pm \num{0.00e+00}$ & $1.89 \pm \num{0.00e+00}$ & $2.51 \pm \num{0.00e+00}$ & $1.84 \pm 0.57$ \\
%     \texttt{kmeans} & $0.06 \pm \num{0.00e+00}$ & $0.06 \pm \num{0.00e+00}$ & $0.05 \pm \num{0.00e+00}$ & $0.06 \pm 0.01$ \\
%     \texttt{sobel} & $0.09 \pm \num{0.00e+00}$ & $0.13 \pm \num{0.00e+00}$ & $0.17 \pm \num{0.00e+00}$ & $0.13 \pm 0.03$ \\
%     \bottomrule
%     \end{tabular}
    
%     \vspace{1em}
%     \begin{tabular}{lllll}
%     \toprule
%     Program & MAML (0) & MAML (1) & MAML (2) & MAML \\
%     \midrule
%     \texttt{fft} & $0.57 \pm 0.18$ & $0.59 \pm 0.19$ & $0.53 \pm 0.14$ & $0.56 \pm 0.17$ \\
%     \texttt{invk2j} & $2.07 \pm 0.63$ & $2.06 \pm 0.59$ & $2.01 \pm 0.56$ & $2.05 \pm 0.57$ \\
%     \texttt{kmeans} & $0.71 \pm 0.43$ & $0.60 \pm 0.37$ & $0.74 \pm 0.50$ & $0.68 \pm 0.42$ \\
%     \texttt{sobel} & $0.24 \pm 0.16$ & $0.18 \pm 0.12$ & $0.25 \pm 0.22$ & $0.22 \pm 0.17$ \\
%     \bottomrule
%     \end{tabular}
    
%     \vspace{1em}
%     \begin{tabular}{lllll}
%     \toprule
%     Program & PTS (0) & PTS (1) & PTS (2) & PTS \\
%     \midrule
%     \texttt{fft} & $0.83 \pm 0.07$ & $0.84 \pm 0.07$ & $0.85 \pm 0.07$ & $0.84 \pm 0.07$ \\
%     \texttt{invk2j} & $2.09 \pm 0.57$ & $2.09 \pm 0.56$ & $2.11 \pm 0.58$ & $2.10 \pm 0.55$ \\
%     \texttt{kmeans} & $0.06 \pm \num{0.00e+00}$ & $0.06 \pm \num{0.00e+00}$ & $0.06 \pm \num{0.00e+00}$ & $0.06 \pm \num{7.58e-04}$ \\
%     \texttt{sobel} & $0.18 \pm \num{0.00e+00}$ & $0.19 \pm \num{0.00e+00}$ & $0.19 \pm \num{0.00e+00}$ & $0.19 \pm \num{3.52e-03}$ \\
%     \bottomrule
%   \end{tabular}
%   \vspace{1em}

%   \begin{tabular}{ll}
%     \toprule
%     Program & RND \\
%     \midrule
%     \texttt{fft} & $0.64 \pm 0.36$ \\
%     \texttt{invk2j} & $2.36 \pm 0.80$ \\
%     \texttt{kmeans} & $0.21 \pm 0.23$ \\
%     \texttt{sobel} & $0.36 \pm 0.34$ \\
%     \bottomrule
%   \end{tabular}
    
%   \caption{
%     Average initial test loss on \textsc{ParrotBenchCPN} for surrogates produced by each initialization method.
%     We include a column for each instance of an initialization method (e.g., ``CPN (0)'' is only one of the \textsc{CompNet}s we trained) as well as a column that averages over each instance (e.g., ``CPN'' is an average over all \textsc{CompNet}s we trained).
%   }\label{fig:parrot_training_time_initial_test_loss}
% \end{figure*}

% \begin{figure*}
%   \begin{tabular}{ll}
%     \toprule
%     Program & RND \\
%     \midrule
%     \texttt{fft} & $\num{3.96e-06}$ \\
%     \texttt{invk2j} & $\num{2.83e-03}$ \\
%     \texttt{kmeans} & $0.01$ \\
%     \texttt{sobel} & $\num{4.16e-04}$ \\
%     \bottomrule
%   \end{tabular}
%   \caption{
%     Target test loss for each \textsc{ParrotBenchCPN} program, set by training randomly initialized surrogates for $5{,}000$ epochs over $9$ trials and using the average final test loss.
%   }\label{fig:parrot_training_time_target_test_loss}
% \end{figure*}


% \begin{figure*}
%   \centering
%   \footnotesize
%   \begin{tabular}{lllll}
%     \toprule
%     Program & CPN-R Z/Z (Clone) (0) & CPN-R Z/Z (Clone) (1) & CPN-R Z/Z (Clone) (2) & CPN-R Z/Z (Clone) \\
%     \midrule
%     \texttt{fft} & $379.7 \pm 31.5$ & $262.0 \pm 15.9$ & $1140.7 \pm 40.3$ & $594.1 \pm 398.0$ \\
%     \texttt{invk2j} & $15000.0 \pm 0.0$ & $9200.7 \pm 885.0$ & $12581.3 \pm 1956.4$ & $12260.7 \pm 2700.6$ \\
%     \texttt{kmeans} & $12.0 \pm 1.5$ & $6.0 \pm 0.0$ & $6.0 \pm 0.0$ & $8.0 \pm 3.0$ \\
%     \texttt{sobel} & $11316.7 \pm 2774.9$ & $10637.0 \pm 2332.6$ & $4232.3 \pm 2168.6$ & $8728.7 \pm 4008.5$ \\
%     \bottomrule
%   \end{tabular}
%   \vspace{1em}

%   \begin{tabular}{lllll}
%     \toprule
%     Program & MAML-Z Z/Z (Reinit) (0) & MAML-Z Z/Z (Reinit) (1) & MAML-Z Z/Z (Reinit) (2) & MAML-Z Z/Z (Reinit) \\
%     \midrule
%     \texttt{fft} & $649.3 \pm 469.7$ & $824.0 \pm 527.4$ & $1069.0 \pm 1047.5$ & $847.4 \pm 722.4$ \\
%     \texttt{invk2j} & $9837.3 \pm 5124.5$ & $5327.7 \pm 4358.9$ & $13949.0 \pm 3153.0$ & $9704.7 \pm 5464.3$ \\
%     \texttt{kmeans} & $198.7 \pm 192.1$ & $13338.7 \pm 4984.0$ & $5018.0 \pm 7486.5$ & $6185.1 \pm 7449.2$ \\
%     \texttt{sobel} & $5695.7 \pm 3764.1$ & $6572.7 \pm 5221.4$ & $3668.3 \pm 2193.8$ & $5312.2 \pm 3970.6$ \\
%     \bottomrule
%   \end{tabular}
%   \vspace{1em}

%   \begin{tabular}{lllll}
%     \toprule
%     Program & PTS (0) & PTS (1) & PTS (2) & PTS \\
%     \midrule
%     \texttt{fft} & $459.3 \pm 241.2$ & $1384.7 \pm 1098.1$ & $1024.3 \pm 1087.0$ & $956.1 \pm 950.3$ \\
%     \texttt{invk2j} & $13794.3 \pm 3345.0$ & $12470.3 \pm 5072.0$ & $6632.7 \pm 5282.7$ & $10965.8 \pm 5477.0$ \\
%     \texttt{kmeans} & $188.0 \pm 36.3$ & $58.7 \pm 42.3$ & $18.3 \pm 1.0$ & $88.3 \pm 80.0$ \\
%     \texttt{sobel} & $9964.0 \pm 4035.9$ & $5436.7 \pm 120.1$ & $7555.7 \pm 485.2$ & $7652.1 \pm 2939.6$ \\
%     \bottomrule
%   \end{tabular}
%   \vspace{1em}

%   \begin{tabular}{ll}
%     \toprule
%     Program & RND \\
%     \midrule
%     \texttt{fft} & $693.0 \pm 689.0$ \\
%     \texttt{invk2j} & $5835.7 \pm 5133.0$ \\
%     \texttt{kmeans} & $5098.7 \pm 7429.2$ \\
%     \texttt{sobel} & $5881.0 \pm 3900.7$ \\
%     \bottomrule
%   \end{tabular}
%   \caption{
%     Average epoch at which each initialization method achieves the target test loss for the training time evaluation on \textsc{ParrotBenchCPN}.
%     We include a column for each instance of an initialization method (e.g., ``CPN (0)'' is only one of the \textsc{CompNet}s we trained) as well as a column that averages over each instance (e.g., ``CPN'' is an average over all \textsc{CompNet}s we trained).
%   }\label{fig:avg_finish_epoch_parrot}
% \end{figure*}

% \begin{figure*}
%   \centering
%   \footnotesize
%     \begin{tabular}{lllll}
%     \toprule
%     Program & CPN (0) & CPN (1) & CPN (2) & CPN \\
%     \midrule
%     \texttt{fft} & $0 / 9$ & $0 / 9$ & $0 / 9$ & $0 / 27$ \\
%     \texttt{invk2j} & $9 / 9$ & $0 / 9$ & $3 / 9$ & $12 / 27$ \\
%     \texttt{kmeans} & $0 / 9$ & $0 / 9$ & $0 / 9$ & $0 / 27$ \\
%     \texttt{sobel} & $0 / 9$ & $0 / 9$ & $0 / 9$ & $0 / 27$ \\
%     \bottomrule
%     \end{tabular}
    
%     \vspace{1em}
%     \begin{tabular}{lllll}
%     \toprule
%     Program & MAML (0) & MAML (1) & MAML (2) & MAML \\
%     \midrule
%     \texttt{fft} & $0 / 9$ & $0 / 9$ & $0 / 9$ & $0 / 27$ \\
%     \texttt{invk2j} & $4 / 9$ & $1 / 9$ & $8 / 9$ & $13 / 27$ \\
%     \texttt{kmeans} & $0 / 9$ & $8 / 9$ & $3 / 9$ & $11 / 27$ \\
%     \texttt{sobel} & $1 / 9$ & $2 / 9$ & $0 / 9$ & $3 / 27$ \\
%     \bottomrule
%     \end{tabular}
    
%     \vspace{1em}
%     \begin{tabular}{lllll}
%     \toprule
%     Program & PTS (0) & PTS (1) & PTS (2) & PTS \\
%     \midrule
%     \texttt{fft} & $0 / 9$ & $0 / 9$ & $0 / 9$ & $0 / 27$ \\
%     \texttt{invk2j} & $7 / 9$ & $7 / 9$ & $1 / 9$ & $15 / 27$ \\
%     \texttt{kmeans} & $0 / 9$ & $0 / 9$ & $0 / 9$ & $0 / 27$ \\
%     \texttt{sobel} & $3 / 9$ & $0 / 9$ & $0 / 9$ & $3 / 27$ \\
%     \bottomrule
%   \end{tabular}
%   \vspace{1em}

%   \begin{tabular}{ll}
%     \toprule
%     Program & RND \\
%     \midrule
%     \texttt{fft} & $0 / 9$ \\
%     \texttt{invk2j} & $0 / 9$ \\
%     \texttt{kmeans} & $3 / 9$ \\
%     \texttt{sobel} & $1 / 9$ \\
%     \bottomrule
%   \end{tabular}

%   \caption{
%     Number of trials where each initialization method does not achieve the target test loss after training for $15{,}000$ epochs during the training time evaluation on \textsc{ParrotBenchCPN}.
%     We include a column for each instance of an initialization method (e.g., ``CPN (0)'' is only one of the \textsc{CompNet}s we trained) as well as a column that sums over each instance (e.g., ``CPN'' is a sum over all \textsc{CompNet}s we trained).
%   }\label{fig:num_timeouts_parrot}
% \end{figure*}

% initial/final loss values (Figures~\ref{fig:final_random_init_surrogate_losses} and \ref{fig:surrogate_initial_losses}) and information used to derive the results in Section~\ref{sec:eval_results} (Figure~\ref{fig:eval_number_of_epochs}).

% In Tables~\ref{tbl:training_time_exestack_test_number_of_epochs} and~\ref{tbl:training_time_parrot_number_of_epochs}, the reported number of epochs is 5001 due to an off-by-one error in how the number of epochs is recorded.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ExeStack Test Result Tables %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{llllllll}
%     \toprule
%       Program & Random & PTS 1 & PTS 2 & PTS 3 & CPN 1 & CPN 2 & CPN 3 \\
%       \midrule
%       3858 & 4247.0 & 4998.0 & 4998.0 & 4998.0 & 1314.0 & 4998.0 & 4998.0 \\
%       379 & 4466.0 & 3897.0 & 4998.0 & 4998.0 & 4998.0 & 4998.0 & 4998.0 \\
%       4141 & 4300.0 & 4998.0 & 4998.0 & 4998.0 & 3654.0 & 2430.0 & 4350.0 \\
%       619 & 4330.0 & 4998.0 & 4998.0 & 4998.0 & 4998.0 & 1742.0 & 3864.0 \\
%       4570 & 3249.0 & 4998.0 & 4998.0 & 4998.0 & 132.0 & 4998.0 & 285.0 \\
%       1708 & 2362.0 & 4998.0 & 4998.0 & 4998.0 & 4998.0 & 4998.0 & 4998.0 \\
%       252 & 4405.0 & 4998.0 & 4998.0 & 4998.0 & 2117.0 & 615.0 & 450.0 \\
%       4046 & 4372.0 & 4998.0 & 4998.0 & 4998.0 & 240.0 & 447.0 & 1272.0 \\
%       4222 & 4372.0 & 4998.0 & 4998.0 & 4998.0 & 1281.0 & 2469.0 & 1191.0 \\
%       2384 & 4001.0 & 4998.0 & 4998.0 & 4998.0 & 801.0 & 381.0 & 96.0 \\
%       \bottomrule
%   \end{tabular}
%   \caption{
%     Number of epochs required for each initialization method to achieve the baseline test error on each of a sample of 10 \textsc{ExeStack} test programs, from the 1,000 we evaluated on.}\label{tbl:training_time_exestack_test_number_of_epochs}
% \end{table*}

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{lll}
%     \toprule
%       Program & Final Baseline Train Loss & Final Baseline Test Loss \\
%       \midrule
%       3858 & $3.7 \times 10^{-6}$ ± $4.1 \times 10^{-7}$ & $3.7 \times 10^{-6}$ ± $4.3 \times 10^{-7}$ \\
%       379 & $1.9 \times 10^{-6}$ ± $4.1 \times 10^{-7}$ & $2.0 \times 10^{-6}$ ± $4.1 \times 10^{-7}$ \\
%       4141 & $3.5 \times 10^{-6}$ ± $3.7 \times 10^{-7}$ & $3.6 \times 10^{-6}$ ± $3.7 \times 10^{-7}$ \\
%       619 & $3.2 \times 10^{-6}$ ± $5.2 \times 10^{-7}$ & $3.5 \times 10^{-6}$ ± $6.3 \times 10^{-7}$ \\
%       4570 & $5.2 \times 10^{-10}$ ± $1.3 \times 10^{-10}$ & $5.2 \times 10^{-10}$ ± $1.3 \times 10^{-10}$ \\
%       1708 & $8.8 \times 10^{-10}$ ± $4.3 \times 10^{-12}$ & $8.8 \times 10^{-10}$ ± $1.7 \times 10^{-12}$ \\
%       252 & $7.6 \times 10^{-5}$ ± $2.7 \times 10^{-5}$ & $7.4 \times 10^{-5}$ ± $2.8 \times 10^{-5}$ \\
%       4046 & $3.5 \times 10^{-6}$ ± $5.1 \times 10^{-7}$ & $3.5 \times 10^{-6}$ ± $5.4 \times 10^{-7}$ \\
%       4222 & $3.5 \times 10^{-6}$ ± $5.1 \times 10^{-7}$ & $3.5 \times 10^{-6}$ ± $5.4 \times 10^{-7}$ \\
%       2384 & $4.7 \times 10^{-6}$ ± $5.4 \times 10^{-7}$ & $4.8 \times 10^{-6}$ ± $6.3 \times 10^{-7}$ \\
%       \bottomrule
%   \end{tabular}
% \end{table*}

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{llllllll}
%       \toprule
%       Program & Random & PTS 1 & PTS 2 & PTS 3 & CPN 1 & CPN 2 & CPN 3 \\
%       \midrule
%       \texttt{invk2j} (0) & 4066.0 & 4998.0 & 4998.0 & 4998.0 & 3083.0 & 4236.0 & 3698.0 \\
%       \texttt{invk2j} (1) & 2914.0 & 4998.0 & 4998.0 & 4998.0 & 3132.0 & 4087.0 & 1768.0 \\
%       \texttt{kmeans} & 117.0 & 898.0 & 268.0 & 460.0 & 138.0 & 101.0 & 181.0 \\
%       \texttt{fft} (1) & 2026.0 & 4998.0 & 4998.0 & 317.0 & 572.0 & 1259.0 & 217.0 \\
%       \texttt{sobel} & 3067.0 & 4998.0 & 4998.0 & 4998.0 & 3119.0 & 4324.0 & 2436.0 \\
%       \texttt{fft} (0) & 751.0 & 658.0 & 4998.0 & 1320.0 & 555.0 & 244.0 & 76.0 \\
%       \bottomrule
%   \end{tabular}
%   \caption{Number of epochs required for neural surrogates produced by each initialization method to achieve the baseline test error on each \textsc{ParrotBenchCPN} program.}\label{tbl:training_time_parrot_number_of_epochs}
% \end{table*}

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{llllllll}
%       \toprule
%       Program & Random & PTS 1 & PTS 2 & PTS 3 & CPN 1 & CPN 2 & CPN 3 \\
%       \midrule
%       \texttt{invk2j} (0) & 1.5 & 1.7 & 1.8 & 1.8 & 1.9 & 1.6 & 1.9 \\
%       \texttt{invk2j} (1) & 6.2 & 4.6 & 4.4 & 4.4 & 4.4 & 3.8 & 3.5 \\
%       \texttt{kmeans} & 0.7 & 0.2 & 0.2 & 0.2 & 0.3 & 0.3 & 0.3 \\
%       \texttt{fft} (1) & 0.7 & 0.7 & 0.7 & 0.7 & 0.6 & 0.4 & 0.6 \\
%       \texttt{sobel} & 0.7 & 0.2 & 0.2 & 0.2 & 0.3 & 0.2 & 0.2 \\
%       \texttt{fft} (0) & 0.5 & 0.9 & 1.0 & 1.0 & 1.6 & 0.5 & 0.4 \\
%       \bottomrule
%   \end{tabular}
%   \caption{Initial train losses for neural surrogates produced by each initialization method on \textsc{ParrotBenchCPN} programs.}\label{tbl:training_time_parrot_init_train_loss}
% \end{table*}

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{llllllll}
%       \toprule
%       Program & Random & PTS 1 & PTS 2 & PTS 3 & CPN 1 & CPN 2 & CPN 3 \\
%       \midrule
%       \texttt{invk2j} (0) & 1.4 & 1.7 & 1.8 & 1.8 & 1.9 & 1.6 & 1.9 \\
%       \texttt{invk2j} (1) & 6.2 & 4.6 & 4.5 & 4.4 & 4.4 & 3.9 & 3.6 \\
%       \texttt{kmeans} & 0.8 & 0.2 & 0.2 & 0.2 & 0.2 & 0.3 & 0.2 \\
%       \texttt{fft} (1) & 0.7 & 0.7 & 0.7 & 0.7 & 0.6 & 0.4 & 0.6 \\
%       \texttt{sobel} & 0.7 & 0.2 & 0.2 & 0.2 & 0.3 & 0.2 & 0.2 \\
%       \texttt{fft} (0) & 0.5 & 0.9 & 1.0 & 1.0 & 1.7 & 0.5 & 0.4 \\
%       \bottomrule
%   \end{tabular}
%   \caption{Initial test losses for neural surrogates produced by each initialization method on \textsc{ParrotBenchCPN} programs.}\label{tbl:training_time_parrot_init_test_loss}
% \end{table*}

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{lll}
%       \toprule
%       Program & Final Baseline Train Loss & Final Baseline Test Loss \\
%       \midrule
%       \texttt{invk2j} (0) & $1.2 \times 10^{-4}$ ± $2.9 \times 10^{-5}$ & $2.1 \times 10^{-4}$ ± $5.4 \times 10^{-5}$ \\
%       \texttt{invk2j} (1) & $9.1 \times 10^{-5}$ ± $2.7 \times 10^{-5}$ & $7.1 \times 10^{-5}$ ± $2.2 \times 10^{-5}$ \\
%       \texttt{kmeans} & $2.1 \times 10^{-6}$ ± $8.4 \times 10^{-7}$ & $4.7 \times 10^{-7}$ ± $2.7 \times 10^{-8}$ \\
%       \texttt{fft} (1) & $1.0 \times 10^{-5}$ ± $7.9 \times 10^{-7}$ & $7.1 \times 10^{-6}$ ± $1.9 \times 10^{-8}$ \\
%       \texttt{sobel} & $4.2 \times 10^{-6}$ ± $4.7 \times 10^{-7}$ & $2.7 \times 10^{-6}$ ± $2.8 \times 10^{-8}$ \\
%       \texttt{fft} (0) & $5.6 \times 10^{-6}$ ± $2.2 \times 10^{-6}$ & $2.3 \times 10^{-6}$ ± $3.4 \times 10^{-7}$ \\
%       \bottomrule
%   \end{tabular}
% \end{table*}


% \begin{figure*}
%   \centering
%   \footnotesize
%   \begin{tabular}{llllll}
%     \toprule
%     Program & RND & CPN-R Z/Z (Clone) (0) & CPN-R Z/Z (Clone) (1) & CPN-R Z/Z (Clone) (2) & CPN-R Z/Z (Clone) \\
%     \midrule
%     \texttt{fft} & $1083.0 \pm 1035.3$ & $819.0 \pm 21.6$ & $405.0 \pm 28.6$ & $2234.0 \pm 63.2$ & $1152.7 \pm 831.4$ \\
%     \texttt{invk2j} & $4353.7 \pm 795.7$ & $5000.0 \pm 0.0$ & $5000.0 \pm 0.0$ & $5000.0 \pm 0.0$ & $5000.0 \pm 0.0$ \\
%     \texttt{kmeans} & $1677.7 \pm 2877.2$ & $13.0 \pm 1.7$ & $6.0 \pm 0.0$ & $6.0 \pm 0.0$ & $8.3 \pm 3.6$ \\
%     \texttt{sobel} & $3873.7 \pm 1052.2$ & $4214.0 \pm 688.6$ & $4670.3 \pm 571.0$ & $2086.0 \pm 1166.6$ & $3656.8 \pm 1402.6$ \\
%     \bottomrule
%     \end{tabular}

%     \vspace{1em}
%     \begin{tabular}{llllll}
%       \toprule
%       Program & RND & MAML-Z Z/Z (Reinit) (0) & MAML-Z Z/Z (Reinit) (1) & MAML-Z Z/Z (Reinit) (2) & MAML-Z Z/Z (Reinit) \\
%       \midrule
%       \texttt{fft} & $1083.0 \pm 1035.3$ & $764.0 \pm 302.5$ & $993.0 \pm 445.2$ & $569.0 \pm 181.5$ & $775.3 \pm 338.3$ \\
%       \texttt{invk2j} & $4353.7 \pm 795.7$ & $5000.0 \pm 0.0$ & $3554.7 \pm 1257.2$ & $5000.0 \pm 0.0$ & $4518.2 \pm 957.8$ \\
%       \texttt{kmeans} & $1677.7 \pm 2877.2$ & $3341.3 \pm 2872.9$ & $3397.3 \pm 2775.9$ & $98.0 \pm 123.9$ & $2278.9 \pm 2582.6$ \\
%       \texttt{sobel} & $3873.7 \pm 1052.2$ & $3849.0 \pm 850.6$ & $3710.7 \pm 1306.3$ & $1971.0 \pm 1133.6$ & $3176.9 \pm 1323.0$ \\
%       \bottomrule
%       \end{tabular}
%       \vspace{1em}

%       \begin{tabular}{llllll}
%         \toprule
%         Program & RND & PTS-R Z/Z (Grow) (0) & PTS-R Z/Z (Grow) (1) & PTS-R Z/Z (Grow) (2) & PTS-R Z/Z (Grow) \\
%         \midrule
%         \texttt{fft} & $1083.0 \pm 1035.3$ & $708.0 \pm 40.6$ & $2113.0 \pm 938.4$ & $2422.7 \pm 2266.4$ & $1747.9 \pm 1459.8$ \\
%         \texttt{invk2j} & $4353.7 \pm 795.7$ & $5000.0 \pm 0.0$ & $5000.0 \pm 0.0$ & $3591.7 \pm 1470.0$ & $4530.6 \pm 1017.9$ \\
%         \texttt{kmeans} & $1677.7 \pm 2877.2$ & $1955.7 \pm 2636.7$ & $1103.0 \pm 1853.3$ & $19.0 \pm 1.7$ & $1025.9 \pm 1817.5$ \\
%         \texttt{sobel} & $3873.7 \pm 1052.2$ & $5000.0 \pm 0.0$ & $4571.0 \pm 171.4$ & $5000.0 \pm 0.0$ & $4857.0 \pm 231.0$ \\
%         \bottomrule
%         \end{tabular}
%   \caption{
%     Average finish epoch by program for training time evaluation.
%     We show averages for each instance of an initialization method, as well as averages over all instances of each initialization method.
%   }
% \end{figure*}



% \begin{figure*}[!ht]
%   \centering
%   \footnotesize
%   \begin{tabular}{llllll}
%     \toprule
%     Program & RND & CPN-R Z/Z (Clone) (0) & CPN-R Z/Z (Clone) (1) & CPN-R Z/Z (Clone) (2) & CPN-R Z/Z (Clone) \\
%     \midrule
%     \texttt{fft} & $1083.0 \pm 1035.3$ & $819.0 \pm 21.6$ & $405.0 \pm 28.6$ & $2234.0 \pm 63.2$ & $1152.7 \pm 831.4$ \\
%     \texttt{invk2j} & $4353.7 \pm 795.7$ & $5000.0 \pm 0.0$ & $5000.0 \pm 0.0$ & $5000.0 \pm 0.0$ & $5000.0 \pm 0.0$ \\
%     \texttt{kmeans} & $1677.7 \pm 2877.2$ & $13.0 \pm 1.7$ & $6.0 \pm 0.0$ & $6.0 \pm 0.0$ & $8.3 \pm 3.6$ \\
%     \texttt{sobel} & $3873.7 \pm 1052.2$ & $4214.0 \pm 688.6$ & $4670.3 \pm 571.0$ & $2086.0 \pm 1166.6$ & $3656.8 \pm 1402.6$ \\
%     \bottomrule
%     \end{tabular}
    
%     \vspace{1em}
%     \begin{tabular}{llllll}
%     \toprule
%     Program & RND & MAML-Z Z/Z (Reinit) (0) & MAML-Z Z/Z (Reinit) (1) & MAML-Z Z/Z (Reinit) (2) & MAML-Z Z/Z (Reinit) \\
%     \midrule
%     \texttt{fft} & $1083.0 \pm 1035.3$ & $764.0 \pm 302.5$ & $993.0 \pm 445.2$ & $569.0 \pm 181.5$ & $775.3 \pm 338.3$ \\
%     \texttt{invk2j} & $4353.7 \pm 795.7$ & $5000.0 \pm 0.0$ & $3554.7 \pm 1257.2$ & $5000.0 \pm 0.0$ & $4518.2 \pm 957.8$ \\
%     \texttt{kmeans} & $1677.7 \pm 2877.2$ & $3341.3 \pm 2872.9$ & $3397.3 \pm 2775.9$ & $98.0 \pm 123.9$ & $2278.9 \pm 2582.6$ \\
%     \texttt{sobel} & $3873.7 \pm 1052.2$ & $3849.0 \pm 850.6$ & $3710.7 \pm 1306.3$ & $1971.0 \pm 1133.6$ & $3176.9 \pm 1323.0$ \\
%     \bottomrule
%     \end{tabular}
    
%     \vspace{1em}
%     \begin{tabular}{llllll}
%     \toprule
%     Program & RND & PTS-R Z/Z (Grow) (0) & PTS-R Z/Z (Grow) (1) & PTS-R Z/Z (Grow) (2) & PTS-R Z/Z (Grow) \\
%     \midrule
%     \texttt{fft} & $1083.0 \pm 1035.3$ & $708.0 \pm 40.6$ & $2113.0 \pm 938.4$ & $2422.7 \pm 2266.4$ & $1747.9 \pm 1459.8$ \\
%     \texttt{invk2j} & $4353.7 \pm 795.7$ & $5000.0 \pm 0.0$ & $5000.0 \pm 0.0$ & $3591.7 \pm 1470.0$ & $4530.6 \pm 1017.9$ \\
%     \texttt{kmeans} & $1677.7 \pm 2877.2$ & $1955.7 \pm 2636.7$ & $1103.0 \pm 1853.3$ & $19.0 \pm 1.7$ & $1025.9 \pm 1817.5$ \\
%     \texttt{sobel} & $3873.7 \pm 1052.2$ & $5000.0 \pm 0.0$ & $4571.0 \pm 171.4$ & $5000.0 \pm 0.0$ & $4857.0 \pm 231.0$ \\
%     \bottomrule
%   \end{tabular}
%   \caption{
%     Average epoch at which each initialization method reaches the target test loss for each benchmark.
%     If an initialization method does not reach the target test loss after 5,000 epochs, we report that it took 5,000 epochs.
%     Each table shows average random initialization results, followed by average results for each instance of a compiler type (e.g., each \textsc{CompNet} we trained), and finally, the average results over all instances of a compiler type (e.g., an average over all \textsc{CompNet}s we trained).
%   }
% \end{figure*}

% \begin{figure*}
%   \centering
%   \scriptsize
%   \begin{tabular}{llllll}
%     \toprule
%     Program & RND & CPN-R Z/Z (Clone) (0) & CPN-R Z/Z (Clone) (1) & CPN-R Z/Z (Clone) (2) & CPN-R Z/Z (Clone) \\
%     \midrule
%     \texttt{fft} & $\num{1.70e-06} \pm \num{1.12e-06}$ & $\num{1.68e-06} \pm \num{8.84e-07}$ & $\num{8.67e-07} \pm \num{2.33e-07}$ & $\num{5.44e-06} \pm \num{2.17e-06}$ & $\num{2.66e-06} \pm \num{2.42e-06}$ \\
%     \texttt{invk2j} & $\num{2.60e-03} \pm \num{1.96e-04}$ & $\num{3.07e-03} \pm \num{4.22e-05}$ & $\num{3.08e-03} \pm \num{4.47e-05}$ & $\num{3.43e-03} \pm \num{6.68e-06}$ & $\num{3.20e-03} \pm \num{1.78e-04}$ \\
%     \texttt{kmeans} & $0.01 \pm 0.01$ & $0.01 \pm \num{1.76e-04}$ & $\num{1.46e-04} \pm \num{3.12e-05}$ & $\num{5.56e-05} \pm \num{2.60e-06}$ & $\num{3.36e-03} \pm \num{4.88e-03}$ \\
%     \texttt{sobel} & $\num{4.90e-04} \pm \num{1.06e-04}$ & $\num{4.96e-04} \pm \num{1.45e-05}$ & $\num{5.52e-04} \pm \num{9.59e-05}$ & $\num{3.93e-04} \pm \num{8.36e-05}$ & $\num{4.80e-04} \pm \num{9.47e-05}$ \\
%     \bottomrule
%     \end{tabular}
    
%     \vspace{1em}
%     \begin{tabular}{llllll}
%     \toprule
%     Program & RND & MAML-Z Z/Z (Reinit) (0) & MAML-Z Z/Z (Reinit) (1) & MAML-Z Z/Z (Reinit) (2) & MAML-Z Z/Z (Reinit) \\
%     \midrule
%     \texttt{fft} & $\num{1.70e-06} \pm \num{1.12e-06}$ & $\num{2.24e-06} \pm \num{1.82e-06}$ & $\num{5.35e-06} \pm \num{5.68e-06}$ & $\num{1.13e-06} \pm \num{9.28e-07}$ & $\num{2.91e-06} \pm \num{3.56e-06}$ \\
%     \texttt{invk2j} & $\num{2.60e-03} \pm \num{1.96e-04}$ & $\num{3.60e-03} \pm \num{1.15e-03}$ & $\num{2.56e-03} \pm \num{3.18e-04}$ & $\num{3.06e-03} \pm \num{1.41e-04}$ & $\num{3.07e-03} \pm \num{7.52e-04}$ \\
%     \texttt{kmeans} & $0.01 \pm 0.01$ & $0.01 \pm 0.01$ & $0.02 \pm 0.01$ & $0.01 \pm 0.01$ & $0.01 \pm 0.01$ \\
%     \texttt{sobel} & $\num{4.90e-04} \pm \num{1.06e-04}$ & $\num{4.40e-04} \pm \num{4.16e-05}$ & $\num{4.23e-04} \pm \num{1.80e-04}$ & $\num{3.24e-04} \pm \num{9.15e-05}$ & $\num{3.96e-04} \pm \num{1.17e-04}$ \\
%     \bottomrule
%     \end{tabular}
    
%     \vspace{1em}
%     \begin{tabular}{llllll}
%     \toprule
%     Program & RND & PTS-R Z/Z (Grow) (0) & PTS-R Z/Z (Grow) (1) & PTS-R Z/Z (Grow) (2) & PTS-R Z/Z (Grow) \\
%     \midrule
%     \texttt{fft} & $\num{1.70e-06} \pm \num{1.12e-06}$ & $\num{2.39e-06} \pm \num{2.19e-06}$ & $\num{8.10e-06} \pm \num{5.72e-06}$ & $\num{2.85e-06} \pm \num{2.34e-06}$ & $\num{4.45e-06} \pm \num{4.28e-06}$ \\
%     \texttt{invk2j} & $\num{2.60e-03} \pm \num{1.96e-04}$ & $\num{3.52e-03} \pm \num{4.26e-04}$ & $\num{3.57e-03} \pm \num{2.54e-04}$ & $\num{2.61e-03} \pm \num{5.05e-04}$ & $\num{3.23e-03} \pm \num{5.88e-04}$ \\
%     \texttt{kmeans} & $0.01 \pm 0.01$ & $0.01 \pm \num{4.32e-04}$ & $\num{3.19e-03} \pm 0.01$ & $\num{1.97e-04} \pm \num{3.17e-05}$ & $\num{4.53e-03} \pm 0.01$ \\
%     \texttt{sobel} & $\num{4.90e-04} \pm \num{1.06e-04}$ & $\num{6.29e-04} \pm \num{7.85e-05}$ & $\num{4.85e-04} \pm \num{6.49e-05}$ & $\num{6.11e-04} \pm \num{2.39e-05}$ & $\num{5.75e-04} \pm \num{8.59e-05}$ \\
%     \bottomrule
%   \end{tabular}
%   \caption{
%     Average test loss each initialization method achieves after 5,000 epochs of training on the full training set for each benchmark.
%     Each table shows average random initialization results, followed by average results for each instance of a compiler type (e.g., each \textsc{CompNet} we trained), and finally, the average results over all instances of a compiler type (e.g., an average over all \textsc{CompNet}s we trained).
%   }
% \end{figure*}



% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{|l|l|l|l|l|l|}
%   \hline
%       Benchmark & Baseline & Random & Hypernet 1 & Hypernet 2 & Hypernet 3 \\ \hline
%       763 & 5001.0 ± 0.0 & 5001.0 ± 0.0 & 5001.0 ± 0.0 & 5001.0 ± 0.0 & 5001.0 ± 0.0 \\ \hline
%       339 & 5001.0 ± 0.0 & 4639.3 ± 511.5 & 5001.0 ± 0.0 & 4219.0 ± 0.0 & 5001.0 ± 0.0 \\ \hline
%       1732 & 5001.0 ± 0.0 & 2766.0 ± 666.3 & 766.0 ± 0.0 & 5001.0 ± 0.0 & 5001.0 ± 0.0 \\ \hline
%       572 & 5001.0 ± 0.0 & 4854.7 ± 123.5 & 43.0 ± 0.0 & 280.0 ± 0.0 & 40.0 ± 0.0 \\ \hline
%       474 & 5001.0 ± 0.0 & 3880.0 ± 1160.1 & 1735.0 ± 0.0 & 1333.0 ± 0.0 & 1678.0 ± 0.0 \\ \hline
%       766 & 5001.0 ± 0.0 & 3914.3 ± 1536.8 & 331.0 ± 0.0 & 244.0 ± 0.0 & 712.0 ± 0.0 \\ \hline
%   \end{tabular}
%   \caption{
%     Number of epochs required for each initialization method to converge to the target test error set by the baseline on \textsc{ExeStack} test programs, averaged over trials.
%   }\label{tbl:training_time_exestack_test_number_of_epochs}
% \end{table*}


% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{|l|l|l|l|l|l|}
%   \hline
%       Benchmark & Baseline & Random & Hypernet 1 & Hypernet 2 & Hypernet 3 \\ \hline
%       763 & 43.2 ± 2.7 & 45.1 ± 1.8 & 50.8 ± 0.0e+00 & 43.6 ± 0.0e+00 & 40.6 ± 0.0e+00 \\ \hline
%       339 & 0.3 ± 0.1 & 0.2 ± 0.1 & 0.3 ± 0.0e+00 & 0.2 ± 0.0e+00 & 0.2 ± 0.0e+00 \\ \hline
%       1732 & 0.2 ± 3.5e-02 & 0.3 ± 0.1 & 1.1e-02 ± 0.0e+00 & 0.2 ± 0.0e+00 & 0.1 ± 0.0e+00 \\ \hline
%       572 & 0.3 ± 0.1 & 0.4 ± 0.3 & 1.1e-02 ± 0.0e+00 & 3.6e-02 ± 0.0e+00 & 9.1e-03 ± 0.0e+00 \\ \hline
%       474 & 0.4 ± 0.1 & 0.5 ± 0.3 & 2.0e-03 ± 0.0e+00 & 2.1e-03 ± 0.0e+00 & 4.9e-04 ± 0.0e+00 \\ \hline
%       766 & 0.4 ± 0.1 & 1.0 ± 0.1 & 3.7e-06 ± 0.0e+00 & 1.0e-05 ± 0.0e+00 & 1.1e-06 ± 0.0e+00 \\ \hline
%   \end{tabular}
%   \caption{
%     Initial train losses for each initialization method on \textsc{ExeStack} test programs, averaged over trials.
%     Note that ``Baseline'' and ``Random'' are the same initialization method.
%   }\label{tbl:training_time_exestack_test_init_train_loss}
% \end{table*}

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{|l|l|l|l|l|l|}
%   \hline
%       Benchmark & Baseline & Random & Hypernet 1 & Hypernet 2 & Hypernet 3 \\ \hline
%       763 & 43.2 ± 2.7 & 45.1 ± 1.8 & 51.1 ± 0.0e+00 & 43.8 ± 0.0e+00 & 40.9 ± 0.0e+00 \\ \hline
%       339 & 0.3 ± 0.1 & 0.2 ± 0.1 & 0.3 ± 0.0e+00 & 0.2 ± 0.0e+00 & 0.2 ± 0.0e+00 \\ \hline
%       1732 & 0.2 ± 3.2e-02 & 0.3 ± 0.1 & 1.1e-02 ± 0.0e+00 & 0.2 ± 0.0e+00 & 0.1 ± 0.0e+00 \\ \hline
%       572 & 0.3 ± 0.1 & 0.4 ± 0.3 & 1.1e-02 ± 0.0e+00 & 3.7e-02 ± 0.0e+00 & 8.8e-03 ± 0.0e+00 \\ \hline
%       474 & 0.4 ± 0.1 & 0.5 ± 0.3 & 2.0e-03 ± 0.0e+00 & 2.0e-03 ± 0.0e+00 & 5.0e-04 ± 0.0e+00 \\ \hline
%       766 & 0.4 ± 0.1 & 1.0 ± 0.1 & 3.9e-06 ± 0.0e+00 & 1.0e-05 ± 0.0e+00 & 1.1e-06 ± 0.0e+00 \\ \hline
%   \end{tabular}
%   \caption{
%     Initial test losses for each initialization method on \textsc{ExeStack} test programs, averaged over trials.
%     Note that ``Baseline'' and ``Random'' are the same initialization method.
%   }\label{tbl:training_time_exestack_test_init_test_loss}
% \end{table*}

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{|l|l|l|}
%   \hline
%       Benchmark & Final Baseline Train Loss & Final Baseline Test Loss \\ \hline
%       763 & 6.1e-05 ± 1.5e-05 & 5.8e-05 ± 1.4e-05 \\ \hline
%       339 & 6.7e-04 ± 2.0e-04 & 6.6e-04 ± 1.7e-04 \\ \hline
%       1732 & 1.7e-06 ± 1.1e-06 & 2.3e-06 ± 1.2e-06 \\ \hline
%       572 & 7.8e-04 ± 1.2e-04 & 6.6e-04 ± 9.4e-05 \\ \hline
%       474 & 2.8e-06 ± 2.6e-06 & 2.9e-06 ± 2.6e-06 \\ \hline
%       766 & 2.2e-09 ± 1.8e-09 & 2.2e-09 ± 1.8e-09 \\ \hline
%   \end{tabular}
% \end{table*}


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % ParrotBenchCPN Result Tables %
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{|l|l|l|l|l|l|}
%   \hline
%       Benchmark & Baseline & Random & Hypernet 1 & Hypernet 2 & Hypernet 3 \\ \hline
%       \texttt{fft} (Output 0) & 5001.0 ± 0.0 & 943.0 ± 241.4 & 1947.0 ± 16.7 & 546.0 ± 6.2 & 193.0 ± 11.2 \\ \hline
%       \texttt{fft} (Output 1) & 5001.0 ± 0.0 & 2376.0 ± 1523.8 & 507.0 ± 5.1 & 1691.0 ± 19.6 & 337.0 ± 2.4 \\ \hline
%       \texttt{invk2j} (Output 0) & 5001.0 ± 0.0 & 3238.7 ± 1246.3 & 2296.0 ± 36.2 & 2290.0 ± 4.2 & 2585.0 ± 6.2 \\ \hline
%       \texttt{invk2j} (Output 1) & 5001.0 ± 0.0 & 311.0 ± 112.6 & 76.0 ± 0.0 & 121.0 ± 0.0 & 85.0 ± 0.0 \\ \hline
%       \texttt{kmeans} & 5001.0 ± 0.0 & 223.0 ± 90.0 & 210.0 ± 3.7 & 474.0 ± 11.3 & 244.0 ± 14.9 \\ \hline
%       \texttt{sobel} & 5001.0 ± 0.0 & 4536.7 ± 358.2 & 3351.0 ± 12.1 & 4993.3 ± 10.8 & 3101.0 ± 3.7 \\ \hline
%   \end{tabular}
%   \caption{
%     Number of epochs required for each initialization method to converge to the target test error set by the baseline on \textsc{ParrotBenchCPN} programs, averaged over trials.
%   }\label{tbl:training_time_parrot_number_of_epochs}
% \end{table*}

% % \begin{figure*}
% %   \centering
% %   \includegraphics*[width=0.75\linewidth]{figures/final_random_init_surrogate_losses}
% %   \caption{Average and standard deviation of loss values achieved by randomly initialized surrogates after training, according to the methodology in Section~\ref{sec:eval_methodology}.}\label{fig:final_random_init_surrogate_losses}
% % \end{figure*}

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{|l|l|l|l|l|l|}
%   \hline
%       Benchmark & Baseline & Random & Hypernet 1 & Hypernet 3 & Hypernet 2 \\ \hline
%       \texttt{fft} (Output 0) & 0.7 ± 0.1 & 0.6 ± 0.3 & 1.7 ± 0.0 & 0.4 ± 0.0 & 0.5 ± 0.0 \\ \hline
%       \texttt{fft} (Output 1) & 0.5 ± 0.0 & 0.7 ± 0.0 & 0.6 ± 0.0 & 0.6 ± 0.0 & 0.4 ± 0.0 \\ \hline
%       \texttt{invk2j} (Output 0) & 1.6 ± 0.1 & 1.8 ± 0.3 & 1.9 ± 0.0 & 1.9 ± 0.0 & 1.5 ± 0.0 \\ \hline
%       \texttt{invk2j} (Output 1) & 5.8 ± 0.8 & 5.6 ± 0.5 & 4.4 ± 0.0 & 3.5 ± 0.0 & 3.8 ± 0.0 \\ \hline
%       \texttt{kmeans} & 0.2 ± 0.1 & 0.5 ± 0.3 & 0.3 ± 0.0 & 0.3 ± 0.0 & 0.3 ± 0.0 \\ \hline
%       \texttt{sobel} & 0.3 ± 0.1 & 0.2 ± 0.1 & 0.3 ± 0.0 & 0.2 ± 0.0 & 0.2 ± 0.0 \\ \hline
%   \end{tabular}
%   \caption{
%     Initial train losses for each initialization method on \textsc{ParrotBenchCPN} programs, averaged over trials.
%     Note that ``Baseline'' and ``Random'' are the same initialization method.
%   }\label{tbl:training_time_parrot_init_train_loss}
% \end{table*}

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{|l|l|l|l|l|l|}
%   \hline
%       Benchmark & Baseline & Random & Hypernet 1 & Hypernet 3 & Hypernet 2 \\ \hline
%       \texttt{fft} (Output 0) & 0.7 ± 0.1 & 0.6 ± 0.3 & 1.7 ± 0.0 & 0.4 ± 0.0 & 0.5 ± 0.0 \\ \hline
%       \texttt{fft} (Output 1) & 0.5 ± 0.0 & 0.7 ± 0.0 & 0.6 ± 0.0 & 0.6 ± 0.0 & 0.4 ± 0.0 \\ \hline
%       \texttt{invk2j} (Output 0) & 1.6 ± 0.1 & 1.8 ± 0.3 & 1.9 ± 0.0 & 1.9 ± 0.0 & 1.5 ± 0.0 \\ \hline
%       \texttt{invk2j} (Output 1) & 5.9 ± 0.8 & 5.6 ± 0.5 & 4.4 ± 0.0 & 3.5 ± 0.0 & 3.8 ± 0.0 \\ \hline
%       \texttt{kmeans} & 0.2 ± 0.1 & 0.5 ± 0.3 & 0.2 ± 0.0 & 0.2 ± 0.0 & 0.3 ± 0.0 \\ \hline
%       \texttt{sobel} & 0.3 ± 0.1 & 0.2 ± 0.1 & 0.3 ± 0.0 & 0.2 ± 0.0 & 0.2 ± 0.0 \\ \hline
%   \end{tabular}
%   \caption{
%     Initial test losses for each initialization method on \textsc{ParrotBenchCPN} programs, averaged over trials.
%     Note that ``Baseline'' and ``Random'' are the same initialization method.
%   }\label{tbl:training_time_parrot_init_test_loss}
% \end{table*}

% \begin{table*}[!ht]
%   \centering
%   \begin{tabular}{|l|l|l|}
%   \hline
%       Benchmark & Final Baseline Train Loss & Final Baseline Test Loss \\ \hline
%       \texttt{fft} (Output 0) & 5.1e-07 ± 3.2e-07 & 6.2e-07 ± 6.7e-07 \\ \hline
%       \texttt{fft} (Output 1) & 6.3e-06 ± 4.1e-06 & 5.2e-06 ± 1.2e-06 \\ \hline
%       \texttt{invk2j} (Output 0) & 2.9e-04 ± 2.1e-04 & 2.7e-04 ± 2.2e-04 \\ \hline
%       \texttt{invk2j} (Output 1) & 1.4e-02 ± 2.0e-02 & 1.4e-02 ± 1.9e-02 \\ \hline
%       \texttt{kmeans} & 1.1e-06 ± 4.4e-07 & 1.9e-07 ± 1.2e-07 \\ \hline
%       \texttt{sobel} & 2.0e-06 ± 3.5e-08 & 2.0e-06 ± 3.8e-07 \\ \hline
%   \end{tabular}
% \end{table*}

% % \begin{figure*}
% %   \centering
% %   \includegraphics*[width=\linewidth]{figures/surrogate_initial_losses}
% %   \caption{Loss values at initialization for both randomly initialized and CompNet-initialized surrogates.}\label{fig:surrogate_initial_losses}
% % \end{figure*}

% % \begin{figure*}
% %   \centering
% %   \includegraphics*[width=\linewidth]{figures/eval_number_of_epochs}
% %   \caption{Average and standard deviation of the number of epochs randomly initialized surrogates were trained for and number of epochs CompNet-initialized surrogates required to match test accuracy.}\label{fig:eval_number_of_epochs}
% % \end{figure*}

